Data2Vis: Automatic Generation of Data Visualizations Using Sequence to Sequence Recurrent Neural Networks

Rapidly creating effective visualizations using expressive grammars is challenging for users who have limited time and limited skills in statistics and data visualization. Even high-level, dedicated visualization tools often require users to manually select among data attributes, decide which transformations to apply, and specify mappings between visual encoding variables and raw or transformed attributes. In this paper we introduce Data2Vis, a neural translation model for automatically generating visualizations from given datasets. We formulate visualization generation as a sequence to sequence translation problem where data specifications are mapped to visualization specifications in a declarative language (Vega-Lite). To this end, we train a multilayered attention-based recurrent neural network (RNN) with long short-term memory (LSTM) units on a corpus of visualization specifications. Qualitative results show that our model learns the vocabulary and syntax for a valid visualization specification, appropriate transformations (count, bins, mean) and how to use common data selection patterns that occur within data visualizations. Data2Vis generates visualizations that are comparable to manually-created visualizations in a fraction of the time, with potential to learn more complex visualization strategies at scale.

==> Makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = paper.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = paper.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< paper.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> background.tex <==

\section{Background}
Background ...

==> evaluation.tex <==
\section{Empirical Evaluation}
To evaluate our model, we explore several metrics that capture notions of success on the automated visualization task. Traditionally, metrics such as BLEU score \cite{Papineni2002} have been used as a  measure of text similarity to evaluate the performance of text generation models. Despite its limitations \cite{reiter2018structured}, this approach works for language translation tasks as it provides a general measure of how well a generated translation overlaps (in meaning) with human generated examples seen in the training set. Given the nature of our target tokens (JSON VegaLite), metrics of content overlap does not provide much information on the qualitation of the generated specification. Furthermore, the concept of a "good" visualization is hard to automatically evaluate, hence the need for meaningful proxies with respect to the task. To this end, we propose two metrics - \textit{language syntax validity} and \textit{visualization syntax validity}. Similar to the BLEU score, we expect these metrics to be used more as a \textit{diagnostic} tool that helps researchers easily weed out bad ideas from good ideas.  

Structured evaluation of BLEU and its limitations https://www.mitpressjournals.org/doi/full/10.1162/coli_a_00322

Language Syntax Validity.
Percentage of generated visualizations that conform to the target visualization language. In our case, this is the percentage of generated specifications that are valid JSON (i.e conform to the JSON language rules and syntax). If the target visualization were in other languages e.g javascript for D3, R for GGPlot, Python for Matplotlib etc, this metric will focus on the percentage of results that conform to javascript, R and Python languages

% LSV = mean( num_valid_json / total_generated_visualizations )

Visualization Syntax Validity .
Percentage of generated visualizations that represent a valid "plotable" visualizations in the target language. For example an invalid visualization may include the use of the wrong primtiive types (e.g. numeric type selected for string variable), incorect transformations (e.g sum appleid to string field).
% VSV = mean( num_valid_vega_spec / total_generated_visualizations )


% Yes. The closect reference is Britz et al [1] where they experiment with various values of beam width and with both unidrectional and bidirectional models to explore its impact on performance (BLEU score) for language translation task.

% Uni vs Bi
% The purpose of comparing models (uni vs bidirectional) is to provide insights on how a bidirectional model may impact performance the task in our use case. Bidirectional models have been shown to improve performance for langauge translation (Britz et al [1]) - we will show if this holds for automatic data visualization tasks.

% Various values of beam width k.
% We compare beam width impact - Britz et al show that a beam width of 5 - 10 provided best BLEU score performance while higher values reduced performance. We will show how beam width impacts performance (using our metrics).

% Why new metrics for evaluation?
% We cannot use BLEU score for evaluation. This is because our tokenisation strategy is character based (not words like in language) and generally not amenable to BLEU definitation. BLEU is a measure of text similarity between generated text translation and references. While we can do this for generated visualizations, it does not have much meaning (e.g. having a higher count/metric similar fieldnames etc does not mean a visualization is better than one with lower count). This inspires our exploration of new metrics that capture how well the model is doing ... e.g. how well it learns the target domain, the visualization language syntax, and use of variables.

Ref
[1] D. Britz, A. Goldie, T. Luong, Q. Le, M.-T. Luong, and Q. Le, “Massive Exploration of Neural Machine Translation Architectures,” ArXiv e-prints, Mar. 2017.

We assembly 100 randomly selected datasets from the RDataset collection with 

bi10.json Json: 0.897 Vega 0.897 Phantom 0.373
uninat5.json Json: 0.96 Vega 0.304 Phantom 0.308
uni10.json Json: 0.898 Vega 0.898 Phantom 0.461
bi5.json Json: 0.826 Vega 0.824 Phantom 0.288
uninat15.json Json: 0.972 Vega 0.588 Phantom 0.326
uni5.json Json: 0.892 Vega 0.772 Phantom 0.434
uni15.json Json: 0.76 Vega 0.696 Phantom 0.421
bi15.json Json: 0.902 Vega 0.901 Phantom 0.32
uninat10.json Json: 0.937 Vega 0.487 Phantom 0.277

-	All models tend to learn the json syntax well
-	Unidireational with attention does better 
-	No attention madel does not learn to use transforms correctly. Instead of selecting from a standard set of transforms (sum, bin etc), it incorrectly uses fieldnames in this section of the visualization, leading to a high number of invalid vegalite

\begin{table*}[]
\centering
\caption{We train 3 model specifications based on attention (with attention vs without attention) and LSTM type (Unidirectional vs Bidirectional) and examine mean performance with multiple values for beam width parameter (k = 5, 10,15,20). Results show that while all models had decent performance on the language validity metric, attention based models consistently outperformed the model without attention on the visualization validity metric. We also observe that the bidirectional model with beam width k = 15 provided the best performance on both metrics. }
\label{tab:modeltable}
\begin{tabular}{p{3.5cm}llllllllllll}
 &  &  &  &  &  &  &  &  &  &  &  &  \\
 & \multicolumn{3}{l}{Beam width (k=5)} & \multicolumn{3}{l}{Beam width (k=10)} & \multicolumn{3}{l}{Beam width (k=15)} & \multicolumn{3}{l}{Beam width (k=20)} \\
 & No Attn & \multicolumn{2}{l}{Attention} & No Attn & \multicolumn{2}{l}{Attention} & No Attn & \multicolumn{2}{l}{Attention} & No Attn & \multicolumn{2}{l}{Attention} \\
Metric & uni & uni & bi & no attn & uni & bi & no attn & uni & bi & no attn & uni & bi \\
Language Validity & 0.960 & 0.892 & 0.826 & 0.937 & 0.898 & 0.897 & 0.967 & 0.760 & 0.901 & 0.97 & 0.838 & 0.878 \\
Visualization Validity & 0.304 & 0.772 & 0.824 & 0.487 & 0.898 & 0.897 & 0.628 & 0.696 & 0.902 & 0.63 & 0.813 & 0.878
\end{tabular}
\end{table*}
